DeepAnalyze: Learning to Localize Crashes at Scale

Crash localization, an important step in debugging crashes, is challenging when dealing with an extremely large number of diverse applications and platforms and underlying root causes. Large-scale error reporting systems, e.g., Windows Error Reporting (WER), commonly rely on manually developed rules and heuristics to localize blamed frames causing the crashes. As new applications and features are routinely introduced and existing applications are run under new environments, developing new rules and maintaining existing ones become extremely challenging. We propose a data-driven solution to address the problem. We start with the first large-scale empirical study of 362K crashes and their blamed methods reported to WER by tens of thousands of applications running in the field. The analysis provides valuable insights on where and how the crashes happen and what methods to blame for the crashes. These insights enable us to develop DeepAnalyze, a novel multi-task sequence labeling approach for identifying blamed frames in stack traces. We evaluate our model with over a million real-world crashes from four popular Microsoft applications and show that DeepAnalyze, trained with crashes from one set of applications, not only accurately localizes crashes of the same applications, but also bootstraps crash localization for other applications with zero to very little additional training data.

==> approach_obsolete.tex <==
\section{Approach}

In this section, we describe in detail, our approach to designing and developing DeepAnalyze. We start by introducing the features used to represent stack frames (Section \ref{sec:model-features}). Next, we describe how \textit{context} is incorporated into our approach by re-imagining crash localization using a novel sequence labeling formulation (Section \ref{sec:sequence-labeling}). Then, we describe the architecture of the multi-task learning based \deepanalyze model (Section \ref{sec:deepanalyze-model}). Lastly, we propose a transfer learning approach to learn and adapt models to newer applications with minimal labeled data (Section \ref{sec:cross-application}).


\begin{table*}
    \caption{Features engineered to represent stack frames for crash localization}
    \label{tab:features}
    \begin{tabular}[t]{lll}
    \toprule
         \textbf{Feature Group} & \textbf{Feature Name} & \textbf{Description} \\
    \midrule
        Semantics & \texttt{namespace} & $n$ dimensional Tf-Idf vector of the namespace\\
            & \texttt{method} & $n$ dimensional Tf-Idf vector of the method\\
    \midrule
        Types of Code & \texttt{is\_appname\_in\_frame} & Does the frame contain the application's name?\\
            & \texttt{is\_first\_app\_frame} & Is it the $1^{st}$ frame with the application's name?\\
            & \texttt{is\_kernel\_code} & Does the frame contain kernel code?\\
            & \texttt{is\_ntdll\_code} & Does the frame contain \texttt{ntdll} code? \todo{rename to is\_core\_module?}\\
            & \texttt{is\_exception\_in\_frame} & Does the frame contain an exception?\\
    \midrule
        Other & \texttt{norm\_frame\_position} & Normalized position of the frame\\
            & \texttt{is\_method\_unknown} & Is the method \texttt{unknown}?\\
            & \texttt{is\_method\_empty} & Is the method empty?\\
            & \texttt{is\_binary\_unknown} & Is the binary \texttt{unknown}?\\
            & \texttt{is\_empty\_frame} & Is the entire frame empty?\\
    \bottomrule
    \end{tabular}
\end{table*}

\subsection{Model Features}
\label{sec:model-features}

Guided by domain expertise and our empirical study, we engineered features shown in Table \ref{tab:features}, for data-driven models. These features transform individual frames in the crash stack into vectors that can be used to learn patterns in data. The features chosen are generic, apply to crashes across applications, and can be grouped into the 3 types briefly described below:

\Paragraph{Semantics:} These features represent the important contents of a frame such as the namespace and method name.Here, we observe that tools such as \banganalyze \cite{glerum2009debugging} utilize a large list of whitelists and heuristics to localize crashes deeper in the stack. Such approaches do not consider the global \textit{semantics} and \textit{relevance} of the function in a frame, i.e., how a function contributes to the crash. To include these semantics, we utilize a simple Term Frequency - Inverse Document Frequency (Tf-Idf) vectorization method \cite{wu2014crashlocator}. With this approach we automatically extract a weighted list of important tokens from namespaces and methods in frames.
    
\Paragraph{Types of Code:} Code from applications (1$st$ and $3rd$ party) are more likely to have bugs and cause crashes, when compared to to kernel code and core OS user-mode code \cite{glerum2009debugging}. To incorporate such information, we use features that check the presence of the application's name in the frame (i.e. the binary name). We also extract features that represent kernel code, core OS modules, and exceptions. These features can help models de-prioritize frames that are less likely to contain the root cause for crashes.
    
\Paragraph{Other Information:} As shown in Section \ref{sec:empirical-analysis}, frames at the top of stacks are more likely to be blamed. We thus utilize the normalized frame position to model how deep in the stack the crash location can be. Also, frames can be incomplete in various scenarios such as some $3rd$ party software, and Linux OS components or standard libraries. To de-prioritize such frames, we use multiple boolean features that check for unknown and missing information in the frame.

By transforming frames using the features described in Table \ref{tab:features}, a stack can now be visualized as a sequence of featurized frames.

\input{Figures/nlp-analogy}

\subsection{Crash Localization as Sequence Labeling}
\label{sec:sequence-labeling}

\textit{Context} is an important aspect of natural language processing (NLP). Natural language communication depends on the use of contextual information to remove ambiguity in content. As a result, solutions to most NLP tasks like language modeling \cite{vaswani2017attention, devlin2018bert}, conversational agents \cite{tian2017make}, and named entity recognition \cite{shetty2021neural}, capture context.

Inspired by this, as shown in Table \ref{tab:seq-labeling}, we draw parallels between NLP and crash dump analysis to identify how context can be incorporated in crash localization models. As shown, an elementary component of NLP is a sentence which can be viewed as a sequence of words. Also, sequence labeling has been well studied in NLP to perform tasks such as Part-of-Speech tagging and Named Entity Recognition \cite{ratnaparkhi1996maximum, li2020survey}. For example, in Table \ref{tab:seq-labeling} the named entity \textit{John} is identified as a \textit{Person} and \textit{Seattle} a \textit{Location}. In NLP, models for sequence labeling consider the entire sequence as input and learn labels for each word using surrounding words to identify patterns.

Similarly, in crash dump analysis, we observe that a stack can be visualized as as a sequence of frames, analogous to a sentence and its constituent words. Also, as shown by our empirical analysis, we find that crash locations often depend on context - frames appearing above and below it. Guided by this, we propose that crash localization can be re-imagined as sequence labeling where we assign each frame a binary category label - \textit{BlameFrame} and  \textit{!BlameFrame}. For example, in Table \ref{tab:seq-labeling}, the third frame ($f_{2}$) is identified as the \textit{BlameFrame} (BF), while the rest are labeled \textit{!BlameFrame} (!BF). Next, we describe the design and architecture of our \deepanalyze model that performs this sequence labeling task.

\input{deepanalyze-model}

\subsection{Cross-Application Crash Localization}
\label{sec:cross-application}

As stated in Section \ref{sec:background}, hardcoding heuristics into code creates challenges with scale and generalizability for unknown future scenarios. Software constantly evolves as new applications, APIs, and programming languages are introduced and become popular. Handling crashes in such new cases usually requires a lot of time and deep domain knowledge to write custom rules and plugins for existing solutions. Here, learning a model instead, can help address the scalability and generalizability challenges with ever growing software.

But, with any supervised machine learning approach, labeled training data is a challenge. For instance, for a new project or application, it is nontrivial to develop accurate crash localization models, as there would be minimal labeled data for training. However, in crashes, we believe that there are many semantics and patterns to be learnt that are common across applications; especially the large portion of frames that represent the underlying system (see Figure~\ref{fig:crashingbinaries}(b)). This implies that models trained on crashes from a global set of applications (source) can be used to localize crashes for a new and disjoint set (target) — \textit{Cross-Application Crash Localization}. 

In this work, we use this to overcome the above mentioned challenges with a \textbf{Transfer Learning} and \textbf{Fine-tuning} approach. Formally, following Pan and Yang \cite{pan2009survey}, transfer learning involves the concepts of a domain and a task. 
A domain $\mathcal{D}$ consists of 2 components; a feature space $\mathcal{X}$ and a marginal probability distribution $P(X)$ where $X = x_1, \dots, x_n \in \mathcal{X}$. 
Given a specific domain, $\mathcal{D} = \{\mathcal{X} , P(X)\}$, a task $\mathcal{T}$ has 2 components; a label space $\mathcal{Y}$ and an objective $f(\cdot)$ (i.e., $T = \{\mathcal{Y}, f(\cdot)\}$), that can be learned from training data. Given this, transfer learning is defined as:

\Paragraph{\textit{Transfer Learning}:} Given a source domain $\mathcal{D}_S$ and learning task $\mathcal{T}_S$, target domain $\mathcal{D}_T$ and learning task $\mathcal{T}_T$, transfer learning aims to improve the learning of the target predictive function $f_T(\cdot)$ in $\mathcal{D}_T$ using the knowledge in $\mathcal{D}_S$ and $\mathcal{T}_S$, where $\mathcal{D}_S \neq \mathcal{D}_T$ , or $\mathcal{T}_S \neq \mathcal{T}_T$.

In our scenario, we observe $\mathcal{D}_S \neq \mathcal{D}_T$, where $\mathcal{D}_S$ is the global set of application crashes and the target $\mathcal{D}_T$ is a new/unseen application's crashes. Specifically, we see that the feature space ($\mathcal{X}$) of the source and target are same, while the marginal probability distributions ($P(X)$) are different. This case is generally known as ``Domain Adaptation'' \cite{daume2006domain}. With that in mind, for cross-application crash localization, we first pre-train a \deepanalyze model on a large dataset of crashes spanning multiple applications (Global model). This model learns general and common information about crashes. Then, for a new application scenario, we transfer the weights of this global model to a new model instance, and fine-tune it to adapt to the application of interest with minimal labeled data. In Section \ref{sec:evaluation}, we test our hypothesis and extensively evaluate this approach by gradually varying the training samples used for fine-tuning.

==> implementation_obsolete.tex <==
\section{implementation}

\deepanalyze and all other machine learning models discussed in this work are implemented in Python 3.7.7, with Keras-2.2.4 and the tensorflow-1.15.0 backend. The semantic vectorizers are implemented using the standard tf-idf vectorizer in scikit-learn. For our Bi-LSTM CRF based models, the length of the sequence is limited to a maximum of 255, as collected by WER. Also, the hidden layer size is set to 200 cells along with a dropout of 25\%. The dropout prevents overfitting by ignoring randomly selected neurons during training.
A major challenge with training neural networks is training it long enough, but not so long that it overfits the training data. To overcome this, we use an early stopping mechanism by stopping training it when the performance of the model on the validation dataset starts to degrade. Lastly, our models are trained on an Ubuntu 16.04 LTS machine, with 24-core Intel Xeon E5-2690 v3 CPU (2.60GHz), 112 GB memory and 64-bit operating system. The machine also has a Nvidia Tesla P100 GPU with 16 GB RAM.


==> overview_obsolete.tex <==
\section{Overview}

Large-scale software systems and products in the field often contain bugs that manifest as crashes, despite massive efforts spent on assuring software quality. But the sheer volume and diversity of crashes in the wild can become overwhelming. Thus, many crash reporting systems \cite{glerum2009debugging, applecrash, mozillacrash} have been deployed to collect and bucketize millions of crashes while developers focus on root causing. 

When a software crashes, often the main sources of information available for debugging are crash stacks \cite{schroter2010stack}. They are not only useful to bucketize crashes \cite{glerum2009debugging, dang2012rebucket}, but also help developers isolate crash locations and arrive at root causes \cite{wu2014crashlocator}. Although crash localization techniques have evolved, many in the field still utilise a large list of handcrafted heuristics \cite{glerum2009debugging, ubuntucrash}. As stated in Section \ref{sec:background}, this creates challenges with managing codebases, scaling, and generalising to newer applications.

Here, we observe the opportunity for data-driven machine learning models. They can learn patterns at a large-scale from past crashes to generalize to future unseen scenarios. In this work, we present \textbf{DeepAnalyze}, a deep learning approach for large-scale crash localization. We frame the crash localization problem as a novel \textit{Sequence Labeling} task. Sequence labeling, well explored in Natural Language Processing (NLP) \cite{nguyen2007comparisons}, involves assigning a categorical label to each member of a sequence of observed values. For example, in Named-Entity Recognition, a sequence labeling task, we locate and label entities in text into predefined categories:

% \vspace{-1em}
\begin{itemize}[label={}, leftmargin=10px]
    \item \textbf{Input}: John lives in Seattle since 2009.
    \item \textbf{Output}: \textbf{[John \textsubscript{PER}]} lives in \textbf{[Seattle \textsubscript{LOC}]} since \textbf{[2003 \textsubscript{YEAR}]}
\end{itemize}

Drawing parallels between NLP and crash dump analysis (Section \ref{sec:sequence-labeling}), we design \deepanalyze to view the crash stack as a sequence of frames, analogous to a sentence and its constituent words. With this approach, we incorporate context of the entire stack for crash localization. Further, \deepanalyze uses a multi-task learning based deep neural network (Section \ref{sec:deepanalyze-model}), that not only leverages information within the stack but also complementary information of higher level problem classes (e.g. Stack Overflow, CPP Exception, Zero Division Error). Below we list some terms used throughout the rest of the paper:

\begin{enumerate}
    \item \textbf{Crash Stack}: Stack traces collected during the crash.
    \item \textbf{Crash Location/Blame Frame}: The frame (and its corresponding method) that most likely caused the crash.
    \item \textbf{Crash Localization/Blame Frame Prediction}: The task of identifying the crash location in the crash stack.
\end{enumerate}

% One simple machine learning approach here is a linear binary classifier (e.g., Logistic Regression) that, given a featurized frame, predicts the likelihood of it being the blame frame. Then, we can pick the most probable frame in a stack as the crash location. Although this approach performs reasonably well (see Section \ref{sec:evaluation}), there are some challenges. Mainly, it assumes that a frame is equally probable to be the crash location, irrespective of the crash scenario and other frames in the stack. That is, it does not consider the crash \textit{context} to make decisions. 

% We further illustrate the importance of context with some examples:

% \textbf{Examples}: Figures \ref{fig:example-stack} (a) and (b), show examples of stacks collected from 2 real Microsoft Edge crashes. The first example is a crash due to a potential bug in the method \texttt{ReleaseDrawTexture} which suspends a rendered UI surface in the browser, before switching to a new one. As illustrated in \ref{fig:example-stack-1}, skipping the top 2 frames that are merely calls to a crash logger, \texttt{ReleaseDrawTexture} is blamed. In the second example, although the larger stack contains similar methods, such as \texttt{ReleaseDrawTexture} (highlighted yellow), the problem is quite different. Here, the crash was caused due to an issue with \texttt{igdi10iumd64} - a user mode Intel graphics driver. In Figure \ref{fig:example-stack-2}, we see that the top 5 frames are graphics driver and Microsoft DirextX methods for handling multimedia tasks. Thus, we blame the topmost method \texttt{igdi10iumd64} based on historic knowledge. This exhibits that whether a frame is the crash location or not, depends significantly on the context of the crash. 
